Religious Mayors, School Appointments, and Teenage Pregnancy

When religious movements win executive office, they can use bureaucratic levers to reshape public services along doctrinal lines. Using a regression discontinuity design on close mayoral elections in Brazil, we show that girls exposed to Pentecostal-party mayors during middle school experience birth rates 40% higher, elevated STD rates, reduced HPV vaccination, and higher dropout rates; older cohorts already past school show no effects. The mechanism operates through personnel: these mayors replace school principals and reduce sexual education in municipal schools by 12.5 percentage points, with no changes in state schools outside their control. No effects emerge from other right-wing parties.

==> tables/tableA_congress_candidates.tex <==
\begin{tabular}{lccc}
\hline\hline
 & Evangelical & Total & Share (\%) \\
 & Candidates & Candidates & \\
\hline
PRB & 30 & 198 & 15.2 \\
PSC & 19 & 135 & 14.1 \\
Other Right-Wing & 32 & 698 &  4.6 \\
PT & 2 & 316 &  0.6 \\
PMDB & 11 & 296 &  3.7 \\
PSDB & 7 & 263 &  2.7 \\
Other Parties & 89 & 3038 &  2.9 \\
\hline
All Parties & 190 & 4944 &  3.8 \\
\hline\hline
\end{tabular}

